A Combinatorial Approach to Rauzy-type Dynamics III: The Sliding Dynamics, Diameter and Algorithm

Rauzy-type dynamics are group actions on a collection of combinatorial objects. The first and best known example (the Rauzy dynamics) concerns an action on permutations, associated to interval exchange transformations (IET) for the Poincar\'e map on compact orientable translation surfaces. The equivalence classes on the objects induced by the group action have been classified by Kontsevich and Zorich in [KZ03] and correspond bijectively to the connected components of the strata of the moduli space of abelian differentials. In a paper [Boi14] Boissy proposed a Rauzy-type dynamics that acts on a subset of the permutations (the standard permutations) and conjectured that the Rauzy classes of this dynamics are exactly the Rauzy classes of the Rauzy dynamics restricted to standard permutations. In this paper, we apply the labelling method introduced in [D18] to classify this dynamics thus proving Boissy's conjecture. Finally, this paper conclude our serie of three papers on the study of the Rauzy dynamics by presenting two new results on the Rauzy classes: An quadratic algorithm for outputting a path between two connected permutations and a tight $\Theta(n)$ bound on the diameter of the Rauzy classes for the alternating distance.

==> pp02_permutdiags.tex <==

%-------------------------------------------------------
\section{Permutational diagram monoids and groups}\label{sec.algsett}
%Definitions}
%-------------------------------------------------------
The labelling method that we introduce in section 2 is a method to classify Rauzy-type dynamics. In this section we define what we mean by Rauzy-type dynamics.

Let $X_I$ be a set of labelled combinatorial objects, with elements
labelled from the set $I$. We shall identify it with the set
$[n]=\{1,2,\ldots,n\}$ (and use the shortcut
%
$X_n \equiv X_{[n]}$).\footnote{The use of $I$ instead of just $[n]$
  is a useful notation when considering substructures: if $x \in X_n$,
  and $x' \subseteq x$ w.r.t.\ some notion of inclusion, it may be
  conventient to say that $x' \in X_I$ for $I$ a suitable subset of
  $[n]$, instead that the canonical one.}
%
The symmetric group $\kS_n$ acts naturally on $X_n$, by producing the
object with permuted labels.

Vertex-labeled graphs (or digraphs, or hypergraphs) are a typical
example.  
Set partitions are a special case of hypergraphs (all vertices have
degree 1).
% , and each label being repeated exactly once).  
Matchings are a special case of partitions, in which all blocks have
size 2.
% (they can be seen as perfect matchings on the complete graph $\cK_{2n}$).  
Permutations $\s$ are a special case of matchings, in which each block
$\{i,j\}$ has $i \in \{1,2,\ldots,n\}$ and $j = \s(i)+n \in
\{n+1,n+2,\ldots,2n\}$.
% (they can be seen as perfect matchings
% on the complete bipartite graph $\cK_{n,n}$).

We will consider dynamics over spaces of this type, generated by
operators of a special form that we now introduce:
\begin{definition}[Monoid and group operators]
\label{def.monoidoperator}
We say that $A$ is a \emph{monoid operator} on set $X_n$, if, for a map $\aa: X_n \to \kS_n$, it consists of the map on $X_n$ defined by
%
\be
A(x) = \aa_{x} x
\ef,
\ee
%
where the action $\aa_x x$ is in the sense of the symmetric-group
action over $X_n$.  We say that $A$ is a \emph{group operator} if,
furthermore, $\aa_{A(x)}=\aa_x$.
\end{definition}
\noindent
Said informally, the function $\aa$ ``poses a question'' to the
structure $x$. The possible answers are different permutations, by which we act on $x$.
Note that is all our applications the set $Y_n=\{\aa_x| x\in X_n\}$ of all possible permutations has a 
much smaller cardinality than $X_n$ and $\kS_n$, i.e.\ very few
`answers' are possible. In the Rauzy case, $|X_n|=|\kS_n|=n!$
while $|Y_n|=n$. The asymptotic behaviour is similar ($|X_n|$ is at
least exponential in $n$, while $|Y_n|$ is linear) in all of our
applications.
\begin{figure}
\begin{center}\includegraphics[scale=.75]{fig_arc_comb_struct_1.pdf}\end{center}
\caption{Let $x\in X_n$ be a combinatorial structure on $n$ vertices. $A_x$ choose a permutation $\s$ depending on $x$ and permutes the vertices of $x$ according to it. We represent this symmetric-group action as a diagrammatic action from below.}
\end{figure}
Clearly we have:

%% W.r.t.\ the generalised diagram operators outlined in the
%% introduction, this is clearly a special case, that may be called
%% \emph{permutational}.  

\begin{proposition}
\label{prop.Groupoperatorsareinvertible}
Group operators are invertible.
\end{proposition}

\pf For a given value of $n$, let $A$ be a group operator on the set
$X_n$.  The property $\aa_{A(x)}=\aa_x$ implies that, for all $k \in \bN$,
$A^k(x) = (\aa_{x})^k x$. Thus, for all $x$ there exists an integer
$d_A(x) \in \bN^+$ such that $A^{d_A(x)}(x)=x$. More precisely,
$d_A(x)$ is (a divisor of) the l.c.m.\ of the cycle-lengths of
$\aa_{x}$. Call
%
$d_A = \lcm_{x \in X_n} d_A(x)$ (i.e., more shortly, the l.c.m.\ over
$y \in Y_n$ of the cycle-lengths of $\alpha_y$). Then $d_A$ is a
finite integer, and we can pose $A^{-1} = A^{d_A-1}$. The reasonings
above show that $A$ is a bijection on $X_n$, and $A^{-1}$ is its
inverse.  \qed

\begin{definition}[monoid and group dynamics]
We call a \emph{monoid dynamics} the datum of a family of spaces
$\{X_n\}_{n \in \bN}$ as above, and a finite collection $\cA=\{A_{i}\}$ of
monoid operators.
We call a \emph{group dynamics} the analogous structure, in which all
$A_i$'s are group operators.

For a monoid dynamics on the datum $S_n = (X_n, \cA)$, we say that 
%
$x, x' \in X_n$ are \emph{strongly connected}, $x \sim x'$, if there
exist words $w, w' \in \cA^*$ such that $w x = x'$ and $w' x' = x$.

For a group dynamics on the datum $S_n = (X_n, \cA)$, we say that $x,
x' \in X_n$ are \emph{connected}, $x \sim x'$, if there exists a word
$w \in \cA^*$ such that $w x = x'$.
% In the two cases, $\sim$ is clearly an equivalence relation.
\end{definition}
\noindent
Here the action $wx$ is in the sense of monoid action.  Being
connected is clearly an equivalence relation, and coincides with the
relation of being graph-connected on the Cayley Graph associated to
the dynamics, i.e.\ the digraph with vertices in $X_n$, and edges $x
\longleftrightarrow_{i} x'$ if $A_i^{\pm 1} x = x'$. An analogous
statement holds for strong-connectivity, and the associated Cayley
Digraph.

We call such dynamics Rauzy-type dynamics since the original Rauzy dynamics that inspired this definition is also of this type. 

%% \footnote{I.e.\ the graph with vertex-set identified
%%   with $X_n$, and edges which are labeled from $\cA \cup \cA^{-1}$ and
%%   oriented: we have the oriented edge $(x,x')$ with label $A$ if
%%   $A(x)=x^{-1}$, and in this case we also have the oriented edge
%%   $(x',x)$ with label $A^{-1}$.}

\begin{definition}[classes of configurations]
Given a dynamics as above, and $x \in X_n$, we define 
%
$C(x) \subseteq X_n$, the \emph{class of $x$}, as the set of
configurations connected to $x$, $C(x)=\{ x' \,:\, x\sim x'\}$.
\end{definition}

We will call those classes the Rauzy classes of the dynamics.

\begin{definition}[Invariant of classes]
Given a dynamics as above, we say that $f: X_n \to G_n$ is an invariant of the dynamics if $f(x)=f(x')$ for every pair $(x,x')$ of connected combinatorial structures.
\end{definition}

Thus given a dynamics $(X_n, \cA)$ our goal is to find a family of invariant $(f_i)$ such that two combinatorial structures are in the same Rauzy class if and only if they have the same invariants.

%\noindent
%Two natural distances on the classes of $X_n$ can be associated to a
%group dynamics with generators $\cA=\{A_i\}$.
%%% The distance is infinite if
%%% two configurations are not in the same class. Then we define.
%\begin{definition}[distance and alternation distance]
%Let $\s$, $\tau$ configurations of $X_n$ in
%the same class. The \emph{graph distance} $d_G(\s,\tau)$ is the
%ordinary graph distance in the associated Cayley Graph,
%i.e.\ $d_G(\s,\tau)$ is the minimum $\ell \in \bN$ such that there
%exists a word $w \in \{A_i,A_i^{-1}\}^*$,
%% $\{L,R,L^{-1},R^{-1}\}^*$, 
%of length $\ell$, such that $\tau = w \s$. A \emph{graph geodesic} is a
%$w$ realising the minimum.  We also define the
%%
%\emph{alternation distance} $d(\s,\tau)$, and 
%%
%\emph{alternation geodesics}, as the analogous quantities, for words
%in the infinite alphabet $\{(A_i)^j\}_{j \geq 1}$.
%%% \footnote{Also in
%%%   the group case, in light of Proposition
%%%   \ref{prop.Groupoperatorsareinvertible} there is no loss of
%%%   generality in taking only $j\geq 1$.}
%%\footnote{I.e., the word $A^7 B^4 C^{-2} A^4$ has length 4.}
%%$\{L^i,R^i\}_{i \geq 1}$.
%\end{definition}
%
%\begin{example}
%If $w = a^3\, b\, a^{-2}\, b^{-3}\, a$, and $w x = x'$, we know that the
%distance $d_G(x,x')$ is at most $3+1+2+3+1=10$, and the alternation
%distance $d(x,x')$ is at most 5.
%\end{example}
%
%\noindent
%Contrarily to graph distance, the alternation distance is stable
%w.r.t.\ a number of combinatorial operations that we will perform on
%our configurations, and which are defined later on in the text or in
%future work (restriction to `primitive classes', study of `reduced
%dynamics', permutations in $\kS_{\infty}$,~\ldots). These facts
%suggests that alternation distance is a more natural notion in this
%family of problems.
%\\[2mm]
% passage to the continuum limit,
%
%\section{Group-decoration}
%
%Now, let $G$ be a finite group, and $X^G_I$ be a set of labeled
%combinatorial objects, such that we have a $G^I$ action, i.e., for
%each element $i \in I$ it is defined a group-action of $G$, over the
%element $i$. As a result, we have a natural group action $\kS_n
%\ltimes G^n$ on $X_n$, which, for $(\s;g_1,\ldots,g_n) \in \kS_n
%\ltimes G^n$, first, for $i=1,\ldots,n$, applies $g_i$ to the $i$-th
%element of the object, and then permutes the objects $i \in I$ with
%the given permutation $\s$ (the fact that we have a semi-direct
%product is easily established).
%
%The notion of monoid and group operators generalises immediately, as
%well as the first few definitions, of classes, distance, etc., that we
%have provided above. Note in particular that, for $A$ to be a group
%operator, we need (as before) that $a(A(x))=a(x)$. However, now the
%$\alpha_a$'s are valued in $\kS_n \ltimes G^n$, instead that in
%$\kS_n$. So for $A$ to be a group operator we need that not only the
%permutation $\s$ is the same for $x$ and for $A(x)$, but also the list
%$(g_1,\ldots,g_n)$ of group-elements in $G^I$. Then, the conclusion of
%Proposition \ref{prop.Groupoperatorsareinvertible} remains valid, and
%the proof requires only minor modifications, in which the orders of
%the group elements $g_i$ enter the l.c.m.  We leave the details to the
%reader.
%
%We mention in passing that the dynamics of $L$ and $R$ introduced in
%the previous section can be described in the `simple' setting
%described in the paragraph above (i.e., with no group $G$). On the
%contrary, the dynamics of $L_c$ and $R_c$ introduced in the previous
%section can be described only in this more general setting, namely
%with the choice $G=\bZ_2$ (an element $g \in \{+1,-1\}$ acts on a
%vertex $i$ by multiplication on the parameter of its adjacent
%edge). However this thesis will not investigate this more general case futher. 
%We will provide more details later on, in Sections ???????  FIX
%THIS !!!
%
%
%\section{The main goal}
%
%The goal of this thesis is to provide \emph{classification theorems}
%for dynamics of this kind.  In particular, we will be concerned with
%the classification of classes, and further combinatorial study of
%their structure, for four special group dynamics: The \emph{Rauzy
%  dynamics}, The \emph{extended Rauzy dynamics}, the \emph{Rauzy
%  dynamics for matching} and the \emph{Involution dynamics for
%  matchings}.
%
%Of these four dynamics, the first two were first introduced by Rauzy
%\cite{Rau79}, and their study was pioneered by Veech \cite{Vee82} (the connected classes are called \emph{Rauzy
%  classes}). In these cases the group action is related to the
%interval exchange map on translation surfaces. Thus, on one side, its
%study is motivated by questions in dynamical systems. On the other
%side, the previously obtained classification of classes relies on
%notions and known results in algebraic geometry.  Section
%\ref{ssec.3families} describes these two dynamics, and Section
%\ref{sec.geome} gives a short account of these connections.
%
%The classification theorems associated to these families have been
%provided (with some \emph{caveat} discussed later on) in a series of
%papers, starting with the seminal work of Kontsevich and Zorich
%\cite{KZ03}, and followed by \cite{Boi12}, so our approach provides
%just an alternative derivation of these results. Nonetheless, it has
%two points of interest.
%
%A first point is that, as our approach is quite different from the
%previous ones, along the way we happen to extract some extra
%information on the combinatorial structure of the Rauzy classes. An
%example, which is mentioned in Section \ref{ssec.surgery_geo_combi},
%is the construction of `many' representatives for each Rauzy class,
%extending previous results of Zorich \cite{Zor08}. 
%%More results of
%%this kind are gathered in section \ref{}.
%
%The second, more methodological point of interest is that our approach
%is completely combinatorial, self-contained, and in particular it
%makes no use of any facts from algebraic geometry. In this sense, it
%answers a question posed by Kontsevich and Zorich in~\cite{KZ03}:
%%
%\begin{quote}
%{\it The extended Rauzy classes can be defined in purely combinatorial
%  terms [...] thus the problem of the description of the extended
%  Rauzy classes, and hence, of the description of connected components
%  of the strata of Abelian differentials, is purely
%  combinatorial. However, it seems very hard to solve it
%  directly. [...] we give a classification of extended Rauzy classes
%  using not only combinatorics but also tools of algebraic geometry,
%  topology and of dynamical systems.}
%\end{quote}
%Note that the task of providing a purely combinatorial proof of these
%classification theorems has been also carried over, with
%% apparently
%different methods than ours, by~\cite{Fic16}.
%
%In the following sections of this thesis, we will address other
%variants of these group actions on combinatorial structures, that, by
%analogy, we name \emph{Rauzy-type dynamics}. However, a number of
%these other versions do not have at the moment any algebraic or
%geometric interpretation. As such the proof employed for the
%classification theorem of the Rauzy dynamics which relies (though it
%does not transpire in the proof) on the underlying geometry of the
%problem (in a way made clear in section \ref{sec.geome}) does not
%generalise.
%
%
%To surmount this difficulty, we develop in section \ref{sec_labelling_method}, a very
%general proof method for the classification theorem of
%\emph{Rauzy-type dynamics} that we call the \emph{labelling
%  method}. Applying the labelling method will provide, in sections
%\ref{chap.invol}, \ref{ch.rauzy2} respectively, a second proof of the
%classification theorem of the Rauzy dynamics as well as proofs of the
%classification theorems of the Involution dynamics for matchings. In section \ref{ch.match} we define the Rauzy dynamics for matchings for which the proof can be carried out and will be in a subsequent paper.
%
%.Finally, we conclude the thesis by presenting a few
%Rauzy-type dynamics for which the labelling method can apply (though
%the method may need some tinkering for a few of those) but that we did
%not solve.
%
%

